Robust and Interpretable Grounding of Spatial References with Relation Networks

Learning representations of spatial references in natural language is a key challenge in tasks like autonomous navigation and robotic manipulation. Recent work has investigated various neural architectures for learning multi-modal representations for spatial concepts. However, the lack of explicit reasoning over entities makes such approaches vulnerable to noise in input text or state observations. In this paper, we develop effective models for understanding spatial references in text that are robust and interpretable, without sacrificing performance. We design a text-conditioned \textit{relation network} whose parameters are dynamically computed with a cross-modal attention module to capture fine-grained spatial relations between entities. This design choice provides interpretability of learned intermediate outputs. Experiments across three tasks demonstrate that our model achieves superior performance, with a 17\% improvement in predicting goal locations and a 15\% improvement in robustness compared to state-of-the-art systems.

==> review.tex <==
\clearpage

\appendix
{\Large\centerline{\textbf{Changes based on previous reviews}}}
\paragraph{Outline.}
We summarize the review, the author response of the previous submission in ACL 2020, and the modification for the current submission.
%
The original paper and the review can be found in the end of the document.

\paragraph{Summary of Major Changes.}
\begin{itemize}
\item We have added substantial discussions on prior work to Introduction and Related Work section to make a connection between our work and prior works.

\item We have revamped the model section to provide more details and clarity. An example is also included in the paper.

\item We have added more details on datasets, experiments, and the ablation studies of the results.

\item We have added new results on robustness and interpretability for ISI and ShapeWorld tasks to provide a detailed analysis of the model.

\item We have added more in-depth discussions about the model to provide the intuition about why the proposed model works in Results Section.
\end{itemize}


\paragraph{Author Response.}
\begin{itemize}

    \item Is it possible to have some more details on the Text Encoder module in Section \ref{sec:model}? 
    
    \textbf{Ans.}: We have rewritten the section for describing the proposed architecture, and provided a running example of using the text encoder module in Appendix \ref{section:implmentation}.  
    
    \item Why does the RL paradigm degrade the performance of the model in almost all the settings considered (Table \ref{table:results})?
    
    \textbf{Ans.}: This is because the RL setting requires better exploration and more interaction with the environment, \ie it is harder than supervised learning of the value maps. 
    %
    We have included the discussion in Section \ref{sec:Overall_performance}.
    
    \item Is the result in Figure \ref{fig:noiseCaseEnv_inter} consistent with other samples in the dataset?
    
    \textbf{Ans.}: Yes, it is consistent with other examples we analyzed.
    %
    We have included more examples in Appendix \ref{appendix:Interpretability}.
    
    \item What is an example of instruction with textual noise?
    
    \textbf{Ans.}: We have included the examples of instruction with textual noise in Figure \ref{fig:noiseCaseEnv_inter} and \ref{fig:noiseCaseEnv}.
    
    \item More in-depth discussion of the method is necessary. For example: Why does it work? When does it fail?
    
    \textbf{Ans.}: We have added more discussions on Section \ref{sec:results} to explain why the model works and when it fails. These include: 
    %
    (1) ablation studies in Appendix \ref{appendix:ablation} to show the importance of using the relation network, 
    %
    (2) visualization of the relation map in Section \ref{sec:results} to investigate how the proposed model process the inputs under the textual or observational noise,
    %
    (3) comparison to the state-of-the-art approach in Section \ref{sec:results} to discuss the difference in terms of the design, and
    %
    (4) discussion of the limitations of the proposed model in Appendix \ref{appendx:weakness} to examine the potential weakness of the model.
    
    \item A discussion on the computational costs (training time, convergence speed) could be helpful.
    
    \textbf{Ans.}: We have included the discussion of computational costs in Appendix \ref{section:implmentation}.  
    
    \item A proper comparison to the related work in cogsci and linguistics.
    
    \textbf{Ans.}: We have added in more discussion on the references, both in introduction and related work sections.
    %
    There is indeed a huge volume of work around spatial reasoning from various angles (\eg cogsci, linguistics, etc.). 
    %
    However, we emphasize that we are operating in the realm of training machine learning models to perform the task (which itself has been the subject of considerable attention recently). 
    %
    Within this context, our goal is to specifically advance neural methods for spatial reasoning while addressing the issues of robustness and interpretability, which has not been attempted in prior work to the best of our knowledge.
    
    \item Details of the parameters.
    
    \textbf{Ans.}: We have added more details of the proposed model in Section \ref{sec:model}, and provided a running example in Appendix \ref{section:implmentation}.  
    
    
    \item Can you provide a definition of the term ``relation'' in the paper?
    
    \textbf{Ans.}: Intuitively, the relation score represents the relevance of the pair of objects (and their positions) in locating the goal. 
    %
    The following max operator allows the model to attend to the pair that has the highest relation score. 
    %
    We have included a clarification of the definition in Section \ref{sec:model}.
    
    \item What was the motivation for the design of the textual and observational noise? 
    
    \textbf{Ans.}: We chose observational noise by adding in irrelevant entities -- this is to test whether the model can hone in only on the objects relevant to the instruction and avoid getting distracted by others. We chose the instructional noise for a similar reason (by adding non-functional words that do not change the semantics of the instruction). %\textbf{Can we cite some similar papers that add noise? this is minor and totally ok if we cannot.}
    
    \item How do we know that the parameter size is not the main reason why the system performs better than~\citet{janner2017representation}?
    
    \textbf{Ans.}: We also experimented with the size of filters in the CNN model of~\citet{janner2017representation} to match the parameters in our model. 
    %
    We found that the baseline performance drops by 5\% since there are too many entities on a single filter.
    %
    This implies that the increase of the parameter size does not have a major impact on the performance.
    
    \item The framework and the model present some critical issues: there are long repetitions, unimportant sections that could be heavily shortened to leave space to the others, and the description of the text encoder module, which is one core component of the proposed architecture, lacks clarity. 

    \textbf{Ans.}:  We have incorporated the suggestions on tightening the paper to make it read better. 
    %
    We have also added in a deeper discussion on the motivation for and challenges of this task.
    %
    In addition, we have rewritten the model section to provide clarity.
    
    \item The paper does not provide enough details on the datasets and the tasks considered
    
    \textbf{Ans.}: We have included the statistics of the dataset in Table \ref{table:dataset} and added more details on each dataset in Appendix \ref{section:stats}.
    
    \item There are no results in ISI and ShapeWorld.
    
    \textbf{Ans.}: We have included the robustness and interpretability analysis on ISI and ShapeWorld in Appendix \ref{section:additionalExp}.
    
\end{itemize}



